Measurement of the production of neighbouring jets in lead-lead collisions at $\sqrt{s_{\mathrm{NN}}} = 2.76$ TeV with the ATLAS detector

This Letter presents measurements of correlated production of nearby jets in Pb+Pb collisions at $\sqrt{s_{\mathrm{NN}}} = 2.76$ TeV using the ATLAS detector at the Large Hadron Collider. The measurement was performed using 0.14 ${\rm nb}^{-1}$ of data recorded in 2011. The production of correlated jet pairs was quantified using the rate, $R_{\Delta R}$, of "neighbouring" jets that accompany "test" jets within a given range of angular distance, $\Delta R$, in the pseudorapidity--azimuthal angle plane. The jets were measured in the ATLAS calorimeter and were reconstructed using the anti-$k_{t}$ algorithm with radius parameters $d = 0.2$, $0.3$, and $0.4$. $R_{\Delta R}$ was measured in different Pb+Pb collision centrality bins, characterized by the total transverse energy measured in the forward calorimeters. A centrality dependence of $R_{\Delta R}$ is observed for all three jet radii with $R_{\Delta R}$ found to be lower in central collisions than in peripheral collisions. The ratios formed by the $R_{\Delta R}$ values in different centrality bins and the values in the 40-80 % centrality bin are presented.

==> macros.tex <==
\newcommand{\nucnuc}{\mbox{A+A}}
\newcommand{\AuAu}{\mbox{Au+Au}}
\newcommand{\PbPb}{\mbox{Pb+Pb}}
\newcommand{\pp}{\mbox{$pp$}}

\RequirePackage{xspace}

\newcommand{\NBJ}{\mbox{$R_{\Delta R}$}}
\newcommand{\Et}{\mbox{$E_{\mathrm{T}}$}}
\newcommand{\ETtest}{\mbox{$E_{\mathrm{T}}^{\mathrm{test}}$}}
\newcommand{\ETtestmin}{\mbox{$E_{\mathrm{T,min}}^{\mathrm{test}}$}}
\newcommand{\ETnbj}{\mbox{$E_{\mathrm{T}}^{\mathrm{nbr}}$}}
\newcommand{\ETnbjmin}{\mbox{$E_{\mathrm{T,min}}^{\mathrm{nbr}}$}}
\newcommand{\Ntest}{\mbox{$N_\mathrm{jet}^{\mathrm{test}}$}}
\newcommand{\Nnbj}{\mbox{$N_\mathrm{jet}^{\mathrm{nbr}}$}}
\newcommand{\Nnbji}{\mbox{$N_{\mathrm{jet},i}^{\mathrm{nbr}}$}}
\newcommand{\ETcombi}{\mbox{$E_{\mathrm{T}}^{\mathrm{comb}}$}}
\newcommand{\ETmerged}{\mbox{$E_{\mathrm{T}}^{\mathrm{merged}}$}}
\newcommand{\dR}{\mbox{$\Delta R$}}
\newcommand{\dRmax}{\mbox{$\Delta R, \mathrm{max}$}}
\newcommand{\RdR}{\mbox{$R_{\Delta R}$}}
\newcommand{\RRdR}{\mbox{$\rho_{R_{\Delta R}}$}}
\newcommand{\RdRmin}{\mbox{$R_{\Delta R, \mathrm{min}}$}}
\newcommand{\RdRmax}{\mbox{$R_{\Delta R, \mathrm{max}}$}}
\newcommand{\test}{test\xspace}
\newcommand{\Test}{test\xspace}
\newcommand{\nearby}{neighbouring\xspace}
\newcommand{\Nearby}{Neighbouring\xspace}
%\newcommand{\avgETtrue}{\mbox{$\langle {E_{\mathrm{T}}}^{\mathrm{jet}}_{\mathrm{true}}\rangle$}}
\newcommand{\avgETtrue}{\mbox{$\langle E_{\mathrm{T}}^{\mathrm{truth}}\rangle$ }}
\newcommand{\ETnbjtrue}{\mbox{$E_{\mathrm{T,truth}}^{\mathrm{nbr}} $}}

\newcommand{\ANpart}{\mbox{$\langle N_{\mathrm{part}}\rangle$}}
\newcommand{\Ncoll}{\mbox{$N_{\mathrm{coll}}$}}
%\newcommand{\Nevt}{\mbox{$N_{\mathrm{evt}}$}}
\newcommand{\Ncone}{\mbox{$N_{\mathrm{cone}}$}}
\newcommand{\Njetcent}{\mbox{$N_{\mathrm{jet}}^{\mathrm{cent}}$}}
\newcommand{\Njet}{\mbox{$N_{\mathrm{jet}}$}}
\newcommand{\Ntrk}{\mbox{$N_{\mathrm{trk}}$}}
\newcommand{\Nch}{\mbox{$N_{\mathrm{ch}}$}}
\newcommand{\NchUE}{\mbox{$N_{\mathrm{ch}}^{\mathrm{UE}}$}}
\newcommand{\nchUE}{\mbox{$n_{\mathrm{ch}}^{\mathrm{UE}}$}}
\newcommand{\Npart}{\mbox{$N_{\mathrm{part}}$}}
\newcommand{\Ntptrt}{N_{\mathrm{2p}}}
\newcommand{\Ntptr}{\mbox{$N_{\mathrm{2p}}$}}
\newcommand{\Nraw}{\mbox{$N^{\mathrm{raw}}$}}
\newcommand{\sqrtsnn}{\mbox{$\sqrt{s_{_\mathrm{NN}}}$}}
\newcommand{\sqrts}{\mbox{$\sqrt{s}$}}
\newcommand{\centrm}{\mathrm{cent}}

\newcommand{\RAA}{\mbox{$R_{\rm AA}$}}
\newcommand{\RFive}{\mbox{$d = 0.5$}}
\newcommand{\RFour}{\mbox{$d = 0.4$}}
\newcommand{\RThree}{\mbox{$d = 0.3$}}
\newcommand{\RTwo}{\mbox{$d = 0.2$}}
\newcommand{\Rcp}{\mbox{$R_{\rm CP}$}}
\newcommand{\Rpc}{\mbox{$R_{\rm PC}$}}
\newcommand{\Sk}{\mbox{$S(k)$}}
\newcommand{\TAA}{\mbox{$T_{\mathrm{AA}}$}}

\newcommand{\antikt}{\mbox{anti-\kt}}
\newcommand{\avgpttrue}{\mbox{$\langle {p_{\mathrm{T}}}^{\mathrm{jet}}_{\mathrm{true}}\rangle$}}
\newcommand{\centup}{^{\mathrm{cent}}}
\newcommand{\deffrel}{\mbox{$\delta \varepsilon/\varepsilon$}}
\newcommand{\ETfcal}{\mbox{$\Sigma E_{\mathrm{T}}^{\mathrm{FCal}}$}}
\newcommand{\eff}{\mbox{$\varepsilon$}}
\newcommand{\fs}{\mbox{${f_{\mathrm{S}}}$}}
\newcommand{\gjet}{\mbox{$\gamma$-jet}}
\newcommand{\invnb}{\mbox{${\rm nb^{-1}}$}}
\newcommand{\invmub}{\mbox{$\mu {\rm b^{-1}}$}}
\newcommand{\kt}{\mbox{$k_{t}$}}
\newcommand{\sumet}{\mbox{$\Sigma E_{\mathrm{T}}$}}
\newcommand{\ETtrue}{\mbox{$E_{\mathrm{T}}^{\mathrm{truth}}$}}
\newcommand{\ETrec}{\mbox{$E_{\mathrm{T}}^{\mathrm{rec}}$}}
%\newcommand{\ETtrue}{\mbox{${E_{\mathrm{T}}}^{\mathrm{jet}}_{\mathrm{true}}$}}
%\newcommand{\ETrec}{\mbox{${E_{{\mathrm{T}}}}^{\mathrm{jet}}_{\mathrm{rec}}$}}
\newcommand{\ETtbyf}{\mbox{$E_{\mathrm{T}}^{3\times 4}$}}
\newcommand{\ETsbys}{\mbox{$E_{\mathrm{T}}^{7\times 7}$}}
\newcommand{\diff}{\mathrm{d}}
\newcommand{\Dphi}{\mbox{$\Delta \phi$}}
\newcommand{\Deta}{\mbox{$\Delta \eta$}}
\newcommand{\DEt}{\mbox{$\Delta \ET$}}
\newcommand{\Dz}{\mbox{$D(z)$}}
\newcommand{\Dzmeas}{\mbox{$D^{\mathrm{meas}}(z)$}}
\newcommand{\Dzsub}{\mbox{$D^{\mathrm{sub}}(z)$}}
\newcommand{\Dpt}{\mbox{$D(\pT)$}}
\newcommand{\Dptmeas}{\mbox{$D^{\mathrm{meas}}(\pT)$}}
\newcommand{\Dptsub}{\mbox{$D^{\mathrm{sub}}(\pT)$}}
\newcommand{\Dptratio}{\mbox{$D(\pT)|_{\mathrm{cent}}/D(\pT)|_{\mathrm{60-80}}$}}
\newcommand{\Dzratio}{\mbox{$D(z)|_{\mathrm{cent}}/D(z)|_{\mathrm{60-80}}$}}
\newcommand{\Delpt}{\mbox{$\Delta \pT$}}
\newcommand{\DRtrk}{\mbox{$\Delta R_{\mathrm{ch}}$}}
\newcommand{\effpteta}{\mbox{$\varepsilon(\pT, \eta)$}}
\newcommand{\effpt}{\mbox{$\varepsilon(\pT)$}}
\newcommand{\phat}{\mbox{$\hat{p}_{\mathrm{T}}$}}
\newcommand{\pthatmin}{\mbox{$\hat{p}^{\mathrm{min}}_{\mathrm{T}}$}}
\newcommand{\pthat}{\mbox{$\hat{p}_{\mathrm{T}}$}}
\newcommand{\etajet}{\mbox{$\eta^{\mathrm{jet}}$}}
\newcommand{\phijet}{\mbox{$\phi^{\mathrm{jet}}$}}
\newcommand{\pTjet}{\mbox{$p_{{\mathrm{T}}}^{\mathrm{jet}}$}}
\newcommand{\pTjetcorr}{\mbox{$p_{{\mathrm{T}}}^{\mathrm{corr}}$}}
\newcommand{\pTch}{\mbox{$p_{{\mathrm{T}}}^{\mathrm{ch}}$}}
\newcommand{\pTtrk}{\mbox{$p_{{\mathrm{T}}}^{\mathrm{trk}}$}}
\newcommand{\pTrec}{\mbox{${p_{{\mathrm{T}}}}^{\mathrm{jet}}_{\mathrm{rec}}$}}
\newcommand{\pTtrue}{\mbox{${p_{\mathrm{T}}}^{\mathrm{jet}}_{\mathrm{true}}$}}
\newcommand{\pTchtrue}{\mbox{${p_{\mathrm{T}}}^{\mathrm{ch}}_{\mathrm{true}}$}}
\newcommand{\pTchrec}{\mbox{${p_{\mathrm{T}}}^{\mathrm{ch}}_{\mathrm{rec}}$}}
\newcommand{\ztrue}{\mbox{$z^{\mathrm{true}}$}}
\newcommand{\zrec}{\mbox{$z^{\mathrm{rec}}$}}
\newcommand{\ptvjet}{\mbox{$\displaystyle {\vec{p}_{\mathrm{T}}}^{\, \mathrm{jet}}$}}
\newcommand{\ptvch} {\mbox{$\displaystyle {\vec{p}_{\mathrm{T}}}^{\, \mathrm{ch}}$}}
\newcommand{\ntrue}{\mbox{$N^{\mathrm{truth}}$}}
\newcommand{\nmatch}{\mbox{$N^{\mathrm{match}}$}}
\newcommand{\rcpcorr}{\mbox{$R_{\mathrm{CP}}$}}
\newcommand{\rcpraw}{\mbox{$R_{\mathrm{CP}}^{\mathrm{meas}}$}}
\newcommand{\unfdn}{_{\mathrm{unf}}}
\newcommand{\xini}{\mbox{$x_{\mathrm{ini}}$}}
\newcommand{\vtwo}{\mbox{$v_2$}}
\newcommand{\Rdz}{\mbox{$R_{D(z)}$}}
\newcommand{\Rdpt}{\mbox{$R_{D(\pT)}$}}
\newcommand{\Rdzmeas}{\mbox{$R_{D(z)}^{\mathrm{meas}}$}}
\newcommand{\Rdptmeas}{\mbox{$R_{D(\pT)}^{\mathrm{meas}}$}}

